Milner's Proof System for Regular Expressions Modulo Bisimilarity is Complete (Crystallization: Near-Collapsing Process Graph Interpretations of Regular Expressions)

Milner (1984) defined a process semantics for regular expressions. He formulated a sound proof system for bisimilarity of process interpretations of regular expressions, and asked whether this system is complete. We report conceptually on a proof that shows that Milner's system is complete, by motivating, illustrating, and describing all of its main steps. We substantially refine the completeness proof by Grabmayer and Fokkink (2020) for the restriction of Milner's system to `1-free' regular expressions. As a crucial complication we recognize that process graphs with empty-step transitions that satisfy the layered loop-existence/elimination property LLEE are not closed under bisimulation collapse (unlike process graphs with LLEE that only have proper-step transitions). We circumnavigate this obstacle by defining a LLEE-preserving `crystallization procedure' for such process graphs. By that we obtain `near-collapsed' process graphs with LLEE whose strongly connected components are either collapsed or of `twin-crystal' shape. Such near-collapsed process graphs guarantee provable solutions for bisimulation collapses of process interpretations of regular expressions.

==> figs/fig-counterex-collapsible.tex <==
\begin{figure*}[!t]
  %
  \begin{flushleft}
    \hspace*{-1.75ex}%
    $
    \begin{aligned}[c]
      \scalebox{0.76}{\input{figs/ex-limit-collapse.tex}}
    \end{aligned}
    %
    \hspace*{-13ex}
    %
    \begin{aligned}[c]
      \scalebox{0.76}{\input{figs/ex-limit-collapse-1.tex}}
    \end{aligned}
    $
  \end{flushleft}
  %
  \vspace*{-2.25ex}
  %
  \caption{\label{fig:countex:collapse}%
           Example of a \protect\LLEEonechart\ $\aonechart$ (on the left) 
                                                            that is not \protect\LLEEpreservingly\ collapsible nor \protect\onecollapsible\
             (see Prop.~\protect\ref{prop:not:LLEE:pres:collapse:minimization},~% 
                        \protect\ref{it:1:prop:not:LLEE:pres:collapse:minimization}). 
             $\aonechart$ has the \protect\LLEEwitness~$\aonecharthat$ 
               that is indicated by colored \protect\loopentry\ transitions (of level~1, green, of level~2, blue).
           The blue and green areas help to recognize $\protect\aonechart$ as a `\protect\twincrystal' 
             with respect to $\protect\aonecharthat$ as defined later in Sect.~\protect\ref{twin-crystals}. 
             $\aonechart$ is not \protect\onebisimulation\ collapsed: %the magenta dashed link relates \protect\onebisimilar\ vertices.\vspace*{-0.75mm}
               the correspondences $\protect\magenta{\protect\dashedmapsto}$ via the `counterpart function $\magenta{\scpfun}$'  
                 indicate a (grounded) functional \protect\onebisimulation\ slice on $\aonechart$.
           The result $\aonecharti{1}$ %$ = \protect\connthroughin{\aonechart}{\bverti{1}}{\bverti{2}}$ 
                                       (on the right)
               of connecting through $\bverti{1}$ to $\bverti{2}$ in $\aonechart$
             is a \protect\onebisimulation\ collapse of $\aonechart$
               that does not satisfy \protect\LEE, and hence cannot\vspace*{-0.75mm} be a \protect\LLEEonechart\ 
               (the indicated \protect\entrybodylabeling~$\aonecharthati{1}$ %$ = \protect\connthroughin{\aonecharthat}{\bverti{1}}{\bverti{2}}$ 
                defines \loopentrytransitions\ but is not a \protect\LLEEwitness).} 
      % \caption{\label{fig:countex:collapse}%
      %          Example of a \protect\LLEEonechart\ whose \protect\onebisimulation\ collapse does not satisfy \protect\LEE, 
      %            nor can it be \protect\onetransition\ refined into a \protect\LLEEonechart,
      %            see Lem.~\ref{lem:limit:collapse}.  
      %          The \protect\LLEEonechart\ $\protect\aonechart$ (on the left) with \protect\LLEEwitness~$\aonecharthat$ 
      %              indicated by colored \protect\loopentry\ transitions (of level~1, green, of level~2, blue),
      %            where $\aonechart$ is not collapsed: the magenta dashed link indicates \protect\onebisimilar\ vertices.\vspace*{-1mm}
      %          The result $\protect\connthroughin{\aonechart}{\bverti{1}}{\bverti{2}}$ (on the right) of connecting through $\bverti{1}$ to $\bverti{2}$ in $\aonechart$
      %            is collapsed, but does not satisfy \protect\LLEE\ (the indicated \protect\entrybodylabeling~$\aonecharthati{1}$ is not a \protect\LLEEwitness), 
      %            nor can it be \protect\onetransition\ refined into a \protect\LLEEonechart.}
  %
\end{figure*}

==> figs/fig-elim-R3-4-2.tex <==
\begin{figure}[t!]
  %
\begin{center}
  %
  \input{figs/elim-R3-4-2.tex}
  %
\end{center}
  %
  \vspace*{-1.5ex}
  \caption{\label{fig:elim:R3.4.2}%
           Illustration of the crucial step for eliminating
             a \protect\precrystalline\ reduced \protect\onebisimilarity\ redundancy $\pair{\bverti{1}}{\bverti{2}}$
             of kind \ref{R3.4.2}: by transforming the underlying \protect\onechart\
               so that $\bverti{1}$ then falls outside of the \protect\scc\ of $\avert$ (which is the \protect\txtloopsbackto\ part of $\avert$).
           For this we use that, due to the form of the given \protect\onebisimilarity\ redundancy of kind \ref{R3.4.2},
             $\avert$ is a substate of $\cverti{1}$ (indicated as magenta dashed arrow left). 
           This fact can be used to redirect every \protect\loopentry\ transition from $\avert$ to
               vertices that are reachable from $\cverti{1}$ by an induced transition.
           This step reduces the size of the \protect\scc\ of $\avert$, because now at least $\bverti{1}$ falls outside of the scc of $\avert$,
             and is in particular no longer reachable from $\avert$.
           As a consequence, $\bverti{1}$ must be \protect\onebisimilar\ 
             to a vertex $y$ in the decreased \scc.         
             In this way a \protect\onebisimilarity\ redundancy $\pair{\bverti{1}}{y}$ and $\pair{\bverti{2}}{y}$ of kind \protect\ref{R1.1}
               arises,
             which can be eliminated by Lem.~\protect\ref{lem:elim:all:but:cryst:1brs}.
           However, $\pair{\cverti{1}}{\cverti{2}}$ remains as a \protect\onebisimilarity\ redundancy of kind \ref{R3.4}
             in the decreased \protect\scc.
           }
\end{figure}
  \afterpage{\FloatBarrier} 

==> figs/fig-insulation-step.tex <==

\begin{figure}[t!]
  % 
  \begin{center}
    % 
    %\scalebox{0.068}{\includegraphics{pics/insulation.jpg}}
    %\input{figs/insulation.tex}
    %
    \vspace*{-2.5ex}
    %
  \end{center}
  %
  \caption{\label{fig:lem:LLEE-preserving:insulation}
           Illustration of an insulation step for
             a loop vertex $\avert$ that is a substate of a vertex~$\bvert$ in its \protect\txtloopsbackto\ part $\protect\sectionto{\avert}{\protect\sloopsbacktortc}$
               (that is, $\avert \isonesubstateof \bvert$ holds, indicated by $\protect\magentadashedLongrightarrow$, and $\bvert\protect\loopsbacktortc\avert$), 
           but not insulated from above (that is, $\avert$ is not \protect\maximalwrt{\protect\sloopsbackto}). 
           The transformation redirects induced transitions from $\avert$ that leave the \protect\txtdescendsinloopto\ part $\sectionfrom{\avert}{\sdescendsinlooptortc}$ of $\avert$
           as proper transitions to \protect\onebisimilar\ targets of induced transitions from $\bvert$ in $\sectionfrom{\avert}{\sdescendsinlooptortc}$.
           In this way, $\avert$ is turned into a loop vertex that is \protect\maximalwrt{\protect\sloopsbackto},
             and that therefore is insulated from above.
            }
  %         
\end{figure}

==> figs/fig-twincrystal-interchange.tex <==
\begin{figure*}[t!]
  %
  \begin{center}
    $
    \begin{aligned}
      \input{figs/fig-twincrystal-interchange-1.tex}
    \end{aligned}
    %
    \qquad
    %
    \begin{aligned}
      \input{figs/fig-twincrystal-interchange-2.tex}
    \end{aligned}
    $
  \end{center}
  %
  \vspace*{-2ex}
  %
  \caption{\label{fig:twincrystal:interchange:schema}%
          Interchanging the roles of top vertex and pivot vertex in a \protect\twincrystal\ by modifying the underlying \protect\LLEEwitness,
          see Prop.~\protect\ref{prop:twincrystal:interchange}.
          The idea is that \loopentry\ transitions from $\toptwinc$ to $\twincpivot$ (drawn very thick blue on the left) 
            are `pushed through' to give rise to \loopentry\ transitions
              from $\pivottwinc$ to $\twinctop$ (drawn very thick green on the right).
          }
  %
\end{figure*} 

==> figs/fig-twincrystals-schema-app.tex <==
\begin{figure}[!t]
  %
\begin{center}
  %
  \begin{aligned}
  %
\end{center}
  %
  \vspace*{-2ex}
  \caption{\label{fig:twin-crystal:schema}%
    Interchanging the roles of top vertex and pivot vertex in a \protect\twincrystal\ by changing the underlying \protect\LLEEwitness~$\aonecharthat$
      into a \protect\LLEEwitness~$\protect\aonecharthatacc$
      by relabeling the \protect\loopentry\ transitions from $\protect\toptwinc$ to $\protect\twincpivot$ into body transitions,
                and the body transitions from $\protect\pivottwinc$ to $\protect\twinctop$ into \protect\loopentry\ transitions 
                using the levels of the removed \protect\loopentry\ transitions.
           }
  %
\end{figure}
